Diffusion Knows Transparency: Repurposing Video Diffusion for Transparent Object Depth and Normal Estimation

Transparent objects remain notoriously hard for perception systems: refraction, reflection and transmission break the assumptions behind stereo, ToF and purely discriminative monocular depth, causing holes and temporally unstable estimates. Our key observation is that modern video diffusion models already synthesize convincing transparent phenomena, suggesting they have internalized the optical rules. We build TransPhy3D, a synthetic video corpus of transparent/reflective scenes: 11k sequences rendered with Blender/Cycles. Scenes are assembled from a curated bank of category-rich static assets and shape-rich procedural assets paired with glass/plastic/metal materials. We render RGB + depth + normals with physically based ray tracing and OptiX denoising. Starting from a large video diffusion model, we learn a video-to-video translator for depth (and normals) via lightweight LoRA adapters. During training we concatenate RGB and (noisy) depth latents in the DiT backbone and co-train on TransPhy3D and existing frame-wise synthetic datasets, yielding temporally consistent predictions for arbitrary-length input videos. The resulting model, DKT, achieves zero-shot SOTA on real and synthetic video benchmarks involving transparency: ClearPose, DREDS (CatKnown/CatNovel), and TransPhy3D-Test. It improves accuracy and temporal consistency over strong image/video baselines, and a normal variant sets the best video normal estimation results on ClearPose. A compact 1.3B version runs at ~0.17 s/frame. Integrated into a grasping stack, DKT's depth boosts success rates across translucent, reflective and diffuse surfaces, outperforming prior estimators. Together, these results support a broader claim: "Diffusion knows transparency." Generative video priors can be repurposed, efficiently and label-free, into robust, temporally coherent perception for challenging real-world manipulation.

==> tables/ablation_inference_steps.tex <==
\begin{table}[!ht]
    \centering
    \caption{Ablation for inference step.}
    \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
        \textbf{\makecell[c]{Inference\\Steps}} & $\text{REL}\downarrow$ & $\text{RMSE}\downarrow$ & $\delta_{1.05}\ \uparrow$  & $\delta_{1.10}\ \uparrow$  & $\delta_{1.25}\ \uparrow$  \\
        \midrule
        30 & 9.87  & \textbf{13.88}  & 36.58 & 63.98 & 92.56 \\ 
        20 & 9.81  & \underline{13.94}  & 36.90 & 64.42 & 92.71 \\ 
        15 & 9.76  & 14.04  & 37.21 & 64.78 & 92.80 \\ 
        10 & \underline{9.74}  & 14.27  & 37.50 & \underline{65.19} & \underline{92.91} \\ 
        5 & \textbf{9.72}  & 14.58  & \textbf{38.17} & \textbf{65.50} & \textbf{93.04} \\ 
        1 & 10.00  & 15.07  & \underline{37.64} & 63.65 & 92.65 \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:inference_step}
\end{table}






% \begin{minipage}{\linewidth} % 用minipage包裹，固定宽度为页面宽
%     \begin{table}[H]
%         \centering
%         \caption{Ablation for inference step.}
%         \resizebox{0.95\columnwidth}{!}{
%         \begin{tabular}{cccccc}
%         \toprule
%             \textbf{\makecell[c]{Inference\\Steps}} & $\text{REL}\downarrow$ & $\text{RMSE}\downarrow$ & $\delta_{1.05}\ \uparrow$  & $\delta_{1.10}\ \uparrow$  & $\delta_{1.25}\ \uparrow$  \\
%             \midrule
%             30 & 9.87  & \textbf{0.1388}  & 36.58 & 63.98 & 92.56 \\ 
%             20 & 9.81  & 0.1394  & 36.90 & 64.42 & 92.71 \\ 
%             15 & 9.76  & 0.1404  & 37.21 & 64.78 & 92.80 \\ 
%             10 & \underline{9.74}  & 0.1427  & 37.50 & 65.19 & 92.91 \\ 
%             5 & \textbf{9.72}  & 0.1458  & \textbf{38.17} & \textbf{65.50} & \textbf{93.04} \\ 
%             1 & 10.00  & 0.1507  & 37.64 & 63.65 & 92.65 \\ 
%             \bottomrule
%         \end{tabular}
%         }
%         \label{tab:inference_step}
%     \end{table}
%     \begin{figure}[H]
%     \includegraphics[width=1\columnwidth]{figures/inference_step_concept.pdf}
%     \label{fig:dataset}
%     \end{figure}
% \end{minipage}
